Painting with Words: Elevating Detailed Image Captioning with Benchmark and Alignment Learning

Image captioning has long been a pivotal task in visual understanding, with recent advancements in vision-language models (VLMs) significantly enhancing the ability to generate detailed image captions. However, the evaluation of detailed image captioning remains underexplored due to outdated evaluation metrics and coarse annotations. In this paper, we introduce DeCapBench along with a novel metric, DCScore, specifically designed for detailed captioning tasks. DCScore evaluates hallucinations and fine-grained comprehensiveness by deconstructing responses into the smallest self-sufficient units, termed primitive information units, and assessing them individually. Our evaluation shows that DCScore aligns more closely with human judgment than other rule-based or model-based metrics. Concurrently, DeCapBench exhibits a high correlation with VLM arena results on descriptive tasks, surpassing existing benchmarks for vision-language models. Additionally, we present an automatic fine-grained feedback collection method, FeedQuill, for preference optimization based on our advanced metric, showing robust generalization capabilities across auto-generated preference data. Extensive experiments on multiple VLMs demonstrate that our method not only significantly reduces hallucinations but also enhances performance across various benchmarks, achieving superior detail captioning performance while surpassing GPT-4o.

==> subtex/_Dep_5experiments_v0.tex <==


\subsection{Experimental Setup}
\paragraph{Model.} 
We present series of LLaVA models \citep{liu2024llava} with different sizes and capabilities for our experiments. We initialize both instruction model and reward model with same parameters as well as same size for validating the effectiveness of our proposed method.

\paragraph{Training Dataset for PPO.} 
To ensure the model learns robust generalization capabilities, diversity in image distributions is crucial. Therefore, we randomly sample images from a wide range of datasets, including MSCOCO \citep{lin2014mscoco}, OpenImages \citep{kuznetsova2020openimages}, and ShareGPT4V \citep{chen2023sharegpt4v}. Additionally, to maintain diversity of instructions during training, we prompt GPT-4o \citep{gpt4o} to generate a variety of caption prompts, and provide in Appendix.

\subsection{Ablations}
\begin{table}[h]
  \centering
    \tablestyle{6pt}{1.1}
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{l|cccccc|c}
    \shline
    \multirow{2}{*}{Train Data} & \multicolumn{7}{c}{Held-Out Eval Dataset} \\
            & HA-DPO & RLHF-V & POVID & CSR & RLAIF-V & STIC & Average \\ \hline
    HA-DPO~\citep{zhao2023hdpo}  &  \color{gray}{93.5}   & 81.1  & 23.7 & 53.5 & 51.0 & 42.0 & 57.5 \\
    RLHF-V~\citep{yu2024rlhfv}  & 82.0   & \color{gray}{94.7} & 30.7 & 44.2 & 48.7 & 67.8 & 61.4\\
    POVID~\citep{zhou2024povid}   & 32.5  & 30.6 & \color{gray}{99.5} & 59.4 & 52.5 & 59.5 & 55.7  \\
    CSR~\citep{zhou2024csr}     & 62.5   & 51.8  & 60.3 & \color{gray}{87.5} & 51.8 & 23.6 & 56.3 \\
    RLAIF-V~\citep{yu2024rlaifv} & 69.5   & 49.5  & 77.6 & 55.5 & \color{gray}{68.1} & 66.8 & 64.5 \\
    STIC~\citep{deng2024stic} & 48.0   & 59.7  & 26.8 & 43.3 & 50.1 & \color{gray}{99.9} & 54.6 \\ \hline
    Ours* & 78.0   & 64.1  & 87.4 & 59.7 & 64.7 & 74.1 & \textbf{71.3} \\
    Ours & 76.5   & 71.9  & 93.2 & 55.2 & 69.4 & 84.9 & \textbf{75.2} \\
    \shline
    \end{tabular}
    }
    \vspace{2ex}
    \caption{Reward model zero-shot accuracy on the held-out validation set trained with different preference data on LLaVA-1.5-7B. * indicates that we only utilize 10k preference data to match the size of other training set.}
    \label{tab:reward_model_acc}
\end{table}


\begin{table}[h]
  \centering
    \tablestyle{6pt}{1.1}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccccccccc}
    \shline
    Method    & MMBench & VizWiz & MMStar & WildVision & LLaVA-W & \datasetname{} & mmHal-V & $\text{CHAIR}_S$ & $\text{CHAIR}_I$ \\ \hline
LLaVA-1.5 &   64.8   &  50.0  &  33.1  &   14.48    &   65.3   &  24.50   & 1.85  &   47.8   &    25.3  \\
+ HA-DPO  &   64.3   &  54.1  &  33.5  &   15.17    &   65.1   &   22.45  &  2.12  &   49.3    &  25.5     \\
+ POVID   &    64.7  &  47.9  &   35.4  &  13.25     &  71.5  &  23.54   &  1.90    &   31.8   &   5.4   \\
+ CSR     &    64.2  &  52.8  &   33.8  &   13.85    &   70.3  &   23.70  &   2.12  &  15.7   &   7.9    \\
+ RLAIF-V &   62.7   &  50.9  &  34.7   &   15.65    &   76.0  &  28.21   &   2.59 &   8.5    &   4.3   \\ \hline
+ Ours    & \textbf{66.3}  &   \textbf{55.2}     &  \textbf{35.8}  &    \textbf{19.68}    &   \textbf{76.0}   &  \textbf{34.52}   &  \textbf{2.60}  &   \textbf{5.1}   &  \textbf{2.6}  \\
    \shline
    \end{tabular}
    }
    \vspace{2ex}
    \caption{The performance of different preference data on LLaVA-1.5-7B across different benchmarks.}
    \label{tab:preference_data_performance}
\end{table}


\paragraph{Preference Data for Reward Model.}
To assess the ability of various preference data to generalize, we trained multiple reward models using the same SFT model. For evaluation, we randomly sampled portions of the preference data that were held out. The findings, presented in Table \ref{tab:reward_model_acc}, reveal that our model achieved the highest accuracy across diverse preference datasets. Notably, with the same scale of training data, our reward model outperformed the human-labeled dataset RLHF-V by 9.9\% in accuracy. It also surpassed the RLAIF-V dataset, which, despite having over 80k training samples, was outperformed by our model that utilized a smaller data size. Additionally, we observed that increasing the amount of training data led to an improvement in average accuracy from 71.3\% to 75.2\%, highlighting the scalability of our approach.


\paragraph{Preference Data for Preference Optimization.}
We delve into how varying types of preference data impact preference optimization. Using LLaVA-1.5-7B as our baseline model, we trained it with a variety of preference datasets. The performance of these models was then assessed through a range of downstream benchmarks in a zero-shot context. As showcased in Table \ref{tab:preference_data_performance}, our approach not only excels in captioning performance but also substantially cuts down on hallucinations, achieving a notable 0.75 improvement on mmHal-V compared to the baseline.


\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/data_scale.pdf}
    \caption{Impact of the preference dataset size. }
    \label{fig:data_scale}
\end{figure}
\paragraph{Data Size.}
We scale up the training set of the reward model, and investigate the correlation between downstream performance through preference optimization. We evaluate different checkpoints ranging from 5,000 to 200,000 training samples, using models of sizes 7B and 13B. The results are illustrated in Figure \ref{fig:data_scale}. As the size of the preference data increased, the performance of mmHal-V improves from 2.05 to 2.6. Similarly, MMStar, which focuses on image understanding, shows a consistent increase from 34.7 to 35.8, yielding a 1.1 point lift. This demonstrates that as the size of preference data for the reward model grows, the model's performance consistently improves since the better reward model provides more accurate signals for preference optimization.


% \begin{wraptable}{r}{.5\textwidth}
\begin{table}[h]
    \centering
    \begin{minipage}{0.52\textwidth}
    \tablestyle{6pt}{1.1}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{l|cccc}
        \shline
        Source of Response & MMStar & LLaVA-W & mmHal-V & \datasetname{} \\ \hline
        Homogeneous & xxxx & xxxx &  xxxx & xxxx  \\
        Heterogeneous & xxxx & xxxx &  xxxx & xxxx  \\
        Homo. + Hetero. & 37.3 & 78.3 &  2.47 & xxxx \\
        \shline
        \end{tabular}
    }
    \vspace{2ex}
    \caption{Comparison of downstream performance across reward models trained with varying sources of preference data.}
    \label{tab:data_source}
    \end{minipage}
    \hfill
    \begin{minipage}{0.44\textwidth}
    \tablestyle{6pt}{1.1}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{l|cccc}
        \shline
        \multirow{2}{*}{Method} & \multicolumn{2}{c}{LLaVA-1.5-7B} & \multicolumn{2}{c}{LLaVA-1.5-13B} \\
            & LLaVA-W & \datasetname{} &  LLaVA-W & \datasetname{} \\
        \hline
        Base & 65.3 & 24.5 & 72.8 & 25.5 \\
        Only $c_p$ & xxxx & xxxx & xxxx & xxxx \\
        Only $c_r$ & xxxx & xxxx & xxxx & xxxx \\
        $c_p$ + $c_r$ & 76.0 & 34.52 & 78.3 & 37.73 \\ \shline
        \end{tabular}
    }
    \vspace{2ex}
    \caption{Ablation of using different reward scores during preference optimization.}
    \label{tab:multi_rewards}
    \end{minipage}

\end{table}

\paragraph{Source of Responses.}
We investigate the impact of the source of model responses within the preference data, considering the hypothesis that improvements may stem from the model's ability to generalize across diverse sources. To test this, we design three experimental settings using LLaVA-1.5-13B. The first setting, dubbed 'Homogeneous,' involves sampling responses exclusively from the same model. The second, 'Heterogeneous,' includes responses from various models such as LLaVA-1.5-7B, LLaVA-1.6-7B, and LLaVA-1.6-13B. The third setting combines responses from both homogeneous and heterogeneous sources. The results are summarized in Table \ref{tab:data_source}.

%  Interestingly, we do not observe any benefit from learning from
% GPT-4V generated responses, in fact, our results suggest that positive samples derived from LLaVA
% 1.5-7B led to a slightly stronger model post alignment


\paragraph{Source of Rewards.}
Table \ref{tab:multi_rewards} provides a comparative analysis of various models by incorporating the preference score for the number of primitive information units ($c_r$) alongside the preference score for the proportion of correct units ($c_p$). We specifically evaluate our method against three distinct variants: (1) the base model without any preference optimization (Base); (2) a model optimized solely with the $c_p$ score (Only $c_p$); and (3) a model optimized exclusively with the $c_r$ score (Only $c_r$). This comparison enables a thorough examination of the impact of each optimization strategy on model performance.


% \paragraph{Relation to Best-of-N.}


% \paragraph{Initialization of Reward Model.}

% \paragraph{Multiple Reward for PPO (Ablate Precision and Recall)}



\subsection{Main Results}
\begin{table}[H]
\centering
\renewcommand{\arraystretch}{1}
    \setlength{\tabcolsep}{2pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|cccccccccccc}
    \toprule
     & \multicolumn{5}{c}{Comprehensive Benchmark} & \multicolumn{4}{c}{Visual Hallucination} & \multicolumn{3}{c}{Visual Chat and Caption} \\
    \cmidrule(lr){2-6}\cmidrule(lr){7-10} \cmidrule(lr){11-13} 
    Method  & MMBench  & MMStar  & TextVQA & VizWiz & SciQA$^{\mathrm{I}}$ & mmHal-V & $\text{CHAIR}_S$ & $\text{CHAIR}_I$ & AMBER & LLaVA-W  & WildVision  & \datasetname{} \\
    \midrule
    \multicolumn{13}{l}{\textit{Proportional Model}}  \\
    \midrule
    GPT-4v & 79.8 & 56.0 & 78.0 & - & 84.6 & 3.83 & 17.1 & 10.1 & 83.4 & 98.0 & 79.8 & 53.44 \\
    \midrule
    \multicolumn{13}{l}{\textit{Model Size: 7B}}  \\
    \midrule
    InstructBLIP  & 36.0  & 30.2  & 34.5 & 50.1 & 60.5 & 1.96 & 19.5 & 11.0 & 76.5 & 60.9  & 5.54  & 21.35 \\
    Qwen-VL  &  60.6  & 37.5  & 61.5 & 38.9 & 68.2 & 2.54 & 40.4 & 20.7 & 81.2 & 67.7  & 17.87  & 19.16 \\
    LLaVA-RLHF$_\text{7B}$  & 51.4  &  34.2  & - & - & - & 2.02 & 38.1 & 18.9 & 79.7 & -  & -  & - \\
    LLaVA-1.5$_\text{7B}$  & 64.8  & 33.1  & 46.1 & 50.0 & 66.8 & 1.85 & 47.8 & 25.3 & 71.5 & 65.3  & 14.48  & 24.50 \\
    ShareGPT4V$_\text{7B}$ & 68.1 & 34.7 & 50.9 & 60.3 & 69.7 & 2.11 & 14.3 & 7.3 & 76.8 & 79.1 & 21.95 & 33.34 \\
    LLaVA-1.6$_\text{7B}$  & 67.1  & 37.6  & 64.9 & 57.6 & 70.2 & 2.58 & 14.9 & 8.3 & 68.0 & 79.8  & 26.15  & 35.74 \\
    CSR$_\text{7B}$  & 64.2  & 33.8  & 45.2 & 54.1 & 70.7 & 2.12 & 15.7 & 7.9 & 73.0 & 70.3  & 13.85  & 23.70 \\
    RLAIF-V$_\text{7B}$  & 62.7  & 34.7  & 44.6 &  50.9 & 68.2 & 2.59 & 8.5 & 4.3 & 54.2 & 76.0  & 15.65  & 28.21 \\
    LLaVA-Onevision$_\text{7B}$ & 80.2  & 61.8  & 76.0 & xxx & 95.9 & xxx & xxxx & xxxx & xxxxx & 81.3 & 54.0  & 43.49 \\

    \midrule
    Ours$_\text{LLaVA-1.5}$  & 66.3  & 35.8  & 45.8 & 55.2 & 68.9 & 2.60 & 5.1 & 2.6 & 79.9 & 76.0  & 19.68  & 34.52 \\
    Ours$_\text{LLaVA-1.6}$  & xxxx  & xxxxx  & xxxx & xxxx & xxxx & xxxx & xxxx & xxxx & xxxxx & xxxxx  & xxxxx  & xxxxxx \\
    Ours$_\text{LLaVA-Onevision}$  & xxxx  & xxxxx  & xxxx & xxxx & xxxx & xxxx & xxxx & xxxx & xxxxx & xxxxx  & xxxxx  & xxxxxx \\


    \midrule
    \multicolumn{13}{l}{\textit{Model Size: 13B}}  \\
    \midrule
    LLaVA-1.5$_\text{13B}$  & 68.7  & 34.3  & 48.7 & 53.6 & 71.6 & 2.33 & 47.8 & 23.2 & 71.3 & 72.8  & 16.17  & 25.55 \\
    LLaVA-1.6$_\text{13B}$  & 69.3  & 40.4  & 66.9 & 60.5 & 73.6 & 2.95 & 13.8 & 7.8 & 72.1 & 85.2  & 33.69  & 36.28 \\
    RLAIF-V$_\text{12B}$ & 68.2  & 40.9  & 62.8 & 70.1 & - & 3.53 & 3.3 & 1.8 & 88.0 & 86.7  & - & 33.32 \\
    \midrule
    Ours$_\text{LLaVA-1.5}$  & 69.2  & 37.3  & 48.5 & 56.8 & 73.4 & 2.47 & 5.7 & 2.8 & 73.8 & 78.3  & xxxxx  & xxxxxx \\
    Ours$_\text{LLaVA-1.6}$  & 70.0  & 41.3  & 66.9 & 64.3 & 73.7 & 3.43 & xxxx & xxxx & xxxxx & xxxxx  & xxxxx  & xxxxxx \\
    \bottomrule
    \end{tabular}%
    }
    \vspace{2ex}
    \caption{Main experimental results of our method and other open-sourced state-of-the-art VLMs.}
    \label{tab:main_exp}
\end{table}

As illustrated in Table \ref{tab:preference_data_performance}, our method consistently outperforms numerous benchmarks. Within the Comprehensive Benchmark category, it achieves state-of-the-art results across various datasets, surpassing most other approaches. Particularly notable is the improvement in datasets related to visual hallucination: mmHal-V scores 2.60, an improvement of 0.75 compared to LLaVA-1.5-7B, while $\text{CHAIR}_S$ and $\text{CHAIR}_I$ exhibit minimal hallucinations at 5.1 and 2.6, respectively, highlighting our model's robustness in reducing false positives. Moreover, our approach demonstrates exceptional performance in visual chat, scoring 76.0 on LLaVA-W. With the incorporation of fine-grained feedback, our method shows significant improvement over LLaVA-1.5-7B and RLAIF-V, showcasing the superiority of our approach.
